Private PAC Learning May be Harder than Online Learning

We continue the study of the computational complexity of differentially private PAC learning and how it is situated within the foundations of machine learning. A recent line of work uncovered a qualitative equivalence between the private PAC model and Littlestone's mistake-bounded model of online learning, in particular, showing that any concept class of Littlestone dimension $d$ can be privately PAC learned using $\mathrm{poly}(d)$ samples. This raises the natural question of whether there might be a generic conversion from online learners to private PAC learners that also preserves computational efficiency. We give a negative answer to this question under reasonable cryptographic assumptions (roughly, those from which it is possible to build indistinguishability obfuscation for all circuits). We exhibit a concept class that admits an online learner running in polynomial time with a polynomial mistake bound, but for which there is no computationally-efficient differentially private PAC learner. Our construction and analysis strengthens and generalizes that of Bun and Zhandry (TCC 2016-A), who established such a separation between private and non-private PAC learner.

==> empirical.tex <==
%!TEX root=main.tex

% We then use the privacy of the learner to show that with $1/poly(n)$
% probability, there exists an $i\in[n],$such that there is a jump
% in the expected value of $h_{r,k,S'}$ evaluated on $x_{i}$ versus
% the expected value of $h_{r,k,S'}$ evaluated on $x_{i+1}$, where $S$ and $S'$ are neighbouring datasets.

% We use $S$ and $S'$ as our challenge messages to break the $\FRE$ security by using the jump as distinguishing advantage. We formalize our statements below.

% We have thus shown that an $(\alpha,\beta)$- accurate learner when given an input a dataset encrypted under a random key, produces a hypothesis which with probability $1/poly(n)$, there exists an $i\in[n],$such that there is a jump
% in the expected value of $h_{r,k,S}$ evaluated on $x_{i}$ versus
% the expected value of $h_{r,k,S}$ evaluated on $x_{i+1}.$ Here,
% the expectation is taken over keys $k$ and the learner $L$ which uses
% $S$ and random tosses $r$ to produce $h_{r,k,S}$.


\begin{lemma}
Let $L$ be an $(\alpha=1/4,\beta=1/4)$ accurate empirical learner for the concept class $\EncThr$ with respect to the data set $S=\left\{ \left(x_{1}=(\params,\Enc(k,m_1)),y_{1}\right),\dots,\left(x_{n}=(\params,\Enc(k,m_n)),y_{n}\right)\right\} $, then there exists an $i\in [n]$ such that $\Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{1}{64n^{2}}$ with probability $\frac{1}{15n}$(where the probability is taken over the random coin tosses of the learner $L$)
\end{lemma}\rathin{$S$ is being encrypted under different keys but the current notation does not describe that}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}
$L$ is an $(\alpha,\beta)$ weak learner where $\alpha$ is the advantage
over random tosses. Accuracy of the empirical learner ensures the following for all $k\in\vert K\vert,$
\begin{align*}
\Pr_{r}\Bigg[\sum_{i=1}^{n}\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i})) & \geq(\frac{1}{2}+\alpha)n\Bigg]\geq1-\beta\\
\Pr_{r}\Bigg[\sum_{i=1}^{n}E_{k}\big[\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i}))\big] & \geq(\frac{1}{2}+\alpha)n\Bigg]\ge1-\beta 
\end{align*}
Note that for a fixed value of $r$ and $i\leq n/2$, $E_{k}\left[\mathds{1}\left(h_{k,r,S}(x_{i})=c_{k}(x_{i})\right)\right]=\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$
and for $i>n/2$, $E_{k}\left[\mathds{1}\left(h_{k,r,S}(x_{i})=c_{k}(x_{i})\right)\right]=1-\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$.
Let $R_{i}=\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$.We can write the
following using the defined notation:
\begin{align*}
\Pr_{r}\left[\sum_{i=1}^{n/2}R_{i}-\sum_{i=n/2+1}^{n}R_{i}\geq\alpha n\right] & \geq1-\beta
\end{align*}
Revisiting the statement, we need to prove the following claim:

$\exists i\in[n]\text{ s.t. }$
\begin{align*}
\Pr_{r}\Bigg[\Big(E_{k}[h_{r,k,S}(x_{i})]-E_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{16\alpha^{2}}{n^{2}}\Bigg] & \geq2/3n
\end{align*}
Assume for the sake of contradiction the given statement is false.
This implies $\forall i\in[n]$
\begin{align*}
\Pr_{r}\Bigg[\Big(E_{k}[h_{r,k,S}(x_{i})]-E_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{16\alpha^{2}}{n^{2}}\Bigg] & <2/3n\\
\Pr_{r}\left[E_{k}[h_{r,k,S}(x_{i})]-E_{k}[h_{r,k,S}(x_{i+1})]\geq\frac{4\alpha}{n}\right] & <2/3n & \text{Probability over smaller support}\\
\Pr_{r}\Bigg[E_{k}[h_{r,k,S}(x_{i})]\geq4\alpha/n+E_{k}[h_{r,k,S}(x_{i+1})]\Bigg] & <2/3n\\
\Pr_{r}\Bigg[\Pr_{k}[h_{r,k,S}(x_{i})=1]\geq4\alpha/n+\Pr_{k}[h_{r,k,S}(x_{i+1})=1]\Bigg] & <2/3n & \text{Using the fact }h:X\rightarrow\left\{ 0,1\right\} \\
\Pr_{r}\left[R_{i}\geq R_{i+1}+4\alpha/n\right] & <2/3n & \text{By definition of \ensuremath{R_{i}=\Pr\left[h_{r,k,S}(x_{i})=1\right]}}\\
\Pr_{r}\left[R_{i}\geq R_{n/2}+4\alpha\left(\frac{n}{2}-i\right)/n\right] & <2/3n & \text{Expressing every \ensuremath{R_{i}}in terms of \ensuremath{R_{n/2}}}\\
\Pr_{r}\left[-R_{n/2+i}\geq-R_{n/2}+4\alpha i/n\right] & <2/3n & \text{Expressing every \ensuremath{R_{n/2+i}} in terms of \ensuremath{R_{n/2}}}\\
\Pr_{r}\text{\ensuremath{\left[\sum_{i=1}^{n/2}R_{i}-\sum_{i=1}^{n/2}R_{n/2+i}\geq\alpha n\right]}} & <2/3 & \text{Using union bound}
\end{align*}
\\
This contradicts the accuracy of the learner when $\beta=1/3$ and
proves the claim that 
\[
\Pr_{r}\Bigg[\Big(E_{k}[h_{r,k,S}(x_{i})]-E_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{16\alpha^{2}}{n^{2}}\Bigg]\geq2/3n
\]
\end{proof}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
$L$ is an $(\alpha,\beta)$- learner. Accuracy of the empirical learner ensures the
following for all $k$ in the keyspace,\rathin{keyspace is not defined. Should i define it?}
\begin{align*}
\Pr_{r}\Bigg[\sum_{i=1}^{n}\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i})) & \geq(1-\alpha)n\Bigg]\geq1-\beta.
\end{align*}
Note that $h$ has two sources of randomness - $k$ and $r$. We wish to bound the accuracy of a learner when evaluated over the same set of plaintexts encrypted under different keys. Formally, we want to lower bound the following:
\begin{align*}
\Pr_{r}\Bigg[\sum_{i=1}^{n}\mathbb{E}_{k}\left[\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i}))\right]\Bigg]
\end{align*}

We use reverse Markov's inequality to bound this. It can be stated as follows:
Let $Z$ be a random variable such that $\Pr[Z\leq a]=1$ for some constant $a$. Then, for any $d< \expt[Z]$,
\begin{equation}\label{eq:rev Markov}
    \Pr[Z>d]\geq \frac{\expt[Z]-d}{a-d}
\end{equation}
Taking expectation over $k$ and $r$, we get,
\begin{align*}
    \underset{r,k}{\expt}\Bigg[\sum_{i=1}^{n}\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i}))\Bigg] & \geq(1-\alpha)(1-\beta)n
\end{align*}

Let $\gamma$ be some value we fix later. Using reverse Markov's inequality \ref{eq:rev Markov} we get,
\[
\begin{aligned}\Pr_{r}\Bigg[\sum_{i=1}^{n}\mathbb{E}_{k}\left[\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i}))\right] & \geq(1-\alpha)(1-\beta)n-\gamma\Bigg]\geq \frac{\gamma}{n-(1-\alpha)(1-\beta)n+\gamma}.\end{aligned}
\]

Fixing $\alpha=\beta=1/4$ and $\gamma=n/32$, we get
\[
\begin{aligned}\Pr_{r}\Bigg[\sum_{i=1}^{n}\mathbb{E}_{k}\left[\mathds{1}(h_{k,r,S}(x_{i})=c_{k}(x_{i}))\right] & \geq\frac{17n}{32}\Bigg]\geq \frac{1}{15}.\end{aligned}
\]

Note that for a fixed value of $r$ and $i\leq n/2$, $\expt_{k}\left[\mathds{1}\left(h_{k,r,S}(x_{i})=c_{k}(x_{i})\right)\right]=\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$
and for $i>n/2$, $\expt_{k}\left[\mathds{1}\left(h_{k,r,S}(x_{i})=c_{k}(x_{i})\right)\right]=1-\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$.
Let $R_{i}=\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$.Using the aforementioned
notation, we get:
\begin{align}\label{eq:jump}
   \Pr_{r}\left[\sum_{i=1}^{n/2}R_{i}-\sum_{i=n/2+1}^{n}R_{i}\geq\frac{n}{32}\right]\geq\frac{1}{15}. 
\end{align}

We will show that there exists an $i\in\left[n\right]$ such that

\begin{align}\label{eq:contra}
\Pr_{r}\Bigg[\Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{1}{64n^{2}}\Bigg] & \geq\frac{1}{15n}.
\end{align}
Assume for the sake of contradiction the given statement (equation \ref{eq:contra}) is false.
This implies that for all $i\in[n]$,
\[
\Pr_{r}\Bigg[\Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{1}{64n^{2}}\Bigg]<\frac{1}{15n}.
\]
\\

Since the set of $r$ for which $\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\geq\frac{1}{8n}$
holds true is a subset of the set of $r$ for which $\Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{1}{64n^{2}}$
holds true, we get the following
\[
\begin{aligned}\frac{1}{15n} & >\Pr_{r}\left[\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\geq\frac{1}{8n}\right]\\
 & =\Pr_{r}\left[\expt_{k}[h_{r,k,S}(x_{i})]\geq\frac{1}{8n}+\expt_{k}[h_{r,k,S}(x_{i+1})]\right]\\
 & =\Pr_{r}\Bigg[\Pr_{k}[h_{r,k,S}(x_{i})=1]\geq\frac{1}{8n}+\Pr_{k}[h_{r,k,S}(x_{i+1})=1]\Bigg] & \text{using the fact that }h:X\rightarrow\left\{ 0,1\right\} \\
 & =\Pr_{r}\left[R_{i}\geq R_{i+1}+\frac{1}{8n}\right] & \text{by definition of }\ensuremath{R_{i}=\Pr\left[h_{r,k,S}(x_{i})=1\right]}
\end{aligned}
\]
\\
Using a union bound over all $i\in [n]$, we get
\[
\Pr_{r}\Bigg[\exists i,R_{i}\geq\frac{1}{8n}+R_{i+1}\Bigg]<\frac{1}{15}.
\]

Taking a complement of the event, it follows that 
\[
\Pr_{r}\Bigg[\forall i,R_{i}<\frac{1}{8n}+R_{i+1}\Bigg]\geq\frac{14}{15}.
\]

It follows that $R_1<\frac{1}{8n}+R_2<\frac{2}{8n}+R_3<\dots <\frac{(n/2)-1}{8n}+R_{n/2}$ and similarly $R_{n/2}>R_{n-1}-\frac{1}{8n}>R_{n-2}-\frac{2}{8n}>\dots >R_{n/2}-\frac{n/2}{8n}$with probability $14/15$. 
Expressing all $R_{i}$ and $R_{n/2+i}$ for $i\in\left[n/2\right]$
in terms of $R_{n/2}$ and summing them up we get, 
\[
\Pr_{r}\text{\ensuremath{\left[\sum_{i=1}^{n/2}R_{i}-\sum_{i=1}^{n/2}R_{n/2+i}<\frac{n}{32}\right]}}\geq\frac{14}{15}.
\]
Taking a complement, we get 
\[
\Pr_{r}\text{\ensuremath{\left[\sum_{i=1}^{n/2}R_{i}-\sum_{i=1}^{n/2}R_{n/2+i}\geq\frac{n}{32}\right]}}<\frac{1}{15}.
\]
\\
This contradicts the statement \ref{eq:jump} and proves our statement.
\end{proof}

% We now construct a set of points $S=\left\{ \left(x_{1}=(\params,\Enc(\sk,m_1)),y_{1}\right),\dots,\left(x_{n}=(\params,\Enc(\sk,m_n)),y_{n}\right)\right\}$
% such that for all $i\in [n]$, there exists a set $R_i$\ containing $O(\log n)$ such that for all $z\in S\backslash R_{i},\Eval(z,x_{i})=\Eval(z,x_{i+1})$. 

We now show how to construct a dataset that follows the `swap log' property. We construct a set $S$ such that for all points
in $S$, we can remove $k\log n$ number of points such that consecutive
points have the same \emph{floor-log distance} with respect to the remaining points in
$S$. Additionally, we show that the \textcolor{red}{swap-log} property of the dataset and the privacy guarantee of the learner permits the hypothesis to distinguish between two consecutive points as seen in \textcolor{red}{Lemma 6.3}.\rathin{Should I use some other symbol for $S$ here?}

TEMP

\begin{lemma}[TEMP]\label{lemma:domain}
Let $N = 2^\ell$ and let $n \le N/4$. Let $P=\left\{ m_i\mid m_{i}=N/2 + 4(i - n/2);0\leq i\leq n \right\}$.
For all $0\le i \le n - 1$, let $B_{i}=\left\{ m_j\mid \exists z\in \mathbb{N} \text{ s.t.\ } \abs{m_{j}-m_{i}}\in\left[2^{z}-8,2^{z}+8\right]\right\}$.
Then (i) $\vert B_i\vert =O(\log n)$, and (ii) for all $m\in P \setminus B_{i}$, $\fld(m,m_{i})=\fld(m,m_{i+1})$.
\end{lemma}

END TEMP

\begin{lemma}\label{lemma:domain}
Let $S=\left\{ m_i\mid m_{i}=4i;0\leq i\leq N/4\right\}$.
For all $0\le i \le |S| - 1$, let $B_{i}=\left\{ m_j\mid \exists z\in \mathbb{N} \text{ s.t.\ } \abs{m_{j}-m_{i}}\in\left[2^{z}-8,2^{z}+8\right]\right\}$.
Then (i) $\vert B_i\vert =O(\log\vert S\vert)$, and (ii) for all $m\in S\backslash B_{i}$, $\fld(m,m_{i})=\fld(m,m_{i+1})$.
\end{lemma}

\begin{proof}
\bun{Propagate simplification of statement to depend only on plaintexts/$\fld$, removal of subscript $t$, through proof}
Consider a point $m_i$ in the set $P$ and consider a point $m$ that belongs to $S\setminus B_i$. Let $p$ be the floor log distance between $m_i$ and $m$. This immediately implies that $\vert m_i-m\vert\leq 2^{p+1}$. By construction of $B_i$, we know that $\vert m_i-m\vert <2^{p+1}-8$. Similarly, $\vert m_i-m\vert >2^{p}+8$.
By the triangle inequality, we know that $\abs{m_{i+1}-m}\leq\abs{m_{i}-m_{i+1}}+\abs{m_{i}-m}<8+2^{p+1}-8=2^{p+1}$.

This implies that $\fld(m_{i+1},m)=p$.

Note that for a fixed point $m_i$, there are only $4$ points in the neighborhood of $2^z$ for a fixed $z$ that are multiples of $4$ i.e. belonging to the set $S$. In the set $S$ which is a subset of $N=[2^l]$, there are only $l$ points that are powers of $2$. In short, the size of $B_i$ is at most $4\log \vert S\vert$. This proves our statement.
\end{proof}


\begin{lemma}
Let $L$ be a $(\alpha=1/4,\beta=1/4)$-accurate and $(\epsilon,\delta)$-private empirical learner for the concept class $\EncThr$ with respect to the data set $S=\left\{ \left(x_{1}=(\params,\Enc(\sk,m_1)),y_{1}\right),\dots,\left(x_{n}=(\params,\Enc(\sk,m_n)),y_{n}\right)\right\} $. Let $i$ be the index of the point such that $\Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq \frac{1}{64n^2}$ with probability $\frac{1}{15n}$. Let $S_i=S\backslash B_i$ where $B_i$ is the set of points defined in Lemma \ref{lemma:domain}. Let the hamming distance between $S$ and $S_i$ be denoted by $s$. Then, $\Big(\expt_{k}[h_{r,k,S_i}(x_{i})]-\expt_{k}[h_{r,k,S_i}(x_{i+1})]\Big)^{2}\geq \frac{1}{64n^2}$ with probability $\frac{e^{-\epsilon}}{15n^c}$ for some constant $c$.
\end{lemma}

TEMP

For every choice of crypto randomness $\vec{r}$, define the following algorithm on message sets: $B_{\vec{r}}(M; r_L) = h_{r_L, \vec{r}, M}$. I claim that differential privacy of the learner $L$ implies that for every $\vec{r}$, the algorithm $B_{\vec{r}}$ is DP. This is because changing one entry of $M$ changes exactly one entry of the dataset that is forwarded to the learner $L$.

Now I claim that the algorithm $A(M; r_L)$ is also DP. This is because $A$ is a postprocessing of  


ALONI's contribution to the temp:

Claim 1: $\exists i,M, \Delta$ st $\Pr_{h,S}[h(x_i) = 0] > \Pr_{h,S}[h(x_{i+1})=0] + \Delta$.

Claim 2 (false): By group privacy: $\Pr_{h,S'}[h(x_i) = 0] > \Pr_{h,S'}[h(x_{i+1})=0] + \Delta'$.

ENDTEMP

\begin{proof}
Consider $A$ as an (inefficient) postprocessing of the learner $L$
as follows: let $A(x_1,\dots x_n)= \Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}$. Define $T$ to
be the set of $r$ for which the output of $A:$ $\Big(\expt_{k}[h_{r,k,S}(x_{i})]-\expt_{k}[h_{r,k,S}(x_{i+1})]\Big)^{2}\geq\frac{1}{64n^{2}}$.
We know for a dataset $S,$ $\Pr\left[A(L(S))\in T\right]\geq 1/15n$.

% We can show that $\Pr\left[A(L(S))\in T\right]=\expt_{f_{a}\sim A}\left[\Pr\left[L(S)\in f_{a}^{-1}\left(T\right)\right]\right]$
% \begin{align*}
% \expt_{f_{a}\sim A}\left[\Pr\left[L(S)\in f_{a}^{-1}\left(T\right)\right]\right] & \leq \expt_{f_{a}\sim A}\left[e^{k'\epsilon}\Pr\left[L(S')\in f_{a}^{-1}\left(T\right)\right]\right]\\
%  & \leq e^{k'\epsilon}\Pr\left[A\left(L(S')\right)\in T\right]
% \end{align*}
Using the post-processing property of differentially private mechanisms, we get that $A\circ L(S)$ is $(\epsilon,\delta)$ differentially private. We switch the input dataset from $S$ to $S_i$ and using group privacy we get,

\begin{align*}
  \Pr\left[A\left(L(S)\right)\in T\right]\leq e^{s\epsilon}\Pr\left[A\left(L(S')\right)\in T\right] + \frac{e^{s\epsilon}-1}{e^\epsilon-1}\cdot\delta
\end{align*}
Since $s=c\log n$ for some constant $c$, we have shown that $\Pr\left[A\left(L(S')\right)\in T\right]\geq\frac{e^{-\epsilon}}{15n^{c'}}$ for some constant $c'.$  
\end{proof} \rathin{can i set $\epsilon$ and $\delta$ to be constants so this looks better?}


We now show how we can design an adversary which uses challenge messages as described in \textcolor{red}{Lemma 6.4} and use the accuracy of the hypothesis as described in textcolor{red}{Lemma 6.3} to distinguish between the challenge messages with non-negligible advantage.
\subsection{Adversary-Challenger Game}
\begin{algorithm}
\label{alg:game}
\begin{enumerate}
\item Set $t=N/2$ and randomly choose $i\in [n]$
\item Let $p_{i}=\left(m_{1},\dots,m_{i-1},m_{i},m_{i+2},\dots m_{n}\right)$
and let $p_{i+1}=\left(m_{1},\dots,m_{i-1},m_{i+1},m_{i+2},\dots,m_{n}\right).$
\item Construct pairs $\left(u^{L},v^{L}\right)$ and $\left(u^{R},v^{R}\right)$
as follows: 
\begin{enumerate}
\item Let $u^{L}=v^{L}=\begin{cases}
p_{i} & \text{w.p. }1/2\\
p_{i+1} & \text{w.p. }1/2
\end{cases}$
\item Let $\begin{cases}
u^{R}=p_{i},v^{R}=p_{i+1} & \text{w.p. }1/2\\
u^{R}=p_{i+1},v^{R}=p_{i} & \text{w.p. }1/2
\end{cases}$
\end{enumerate}
\item Challenger samples two random keys $k_{u}$ and $k_{v}$ and sends
back adversary $c_{u}=\Enc(k_{u},u^{b}),c_{v}=\Enc(k_{v},v^{b})$
for $b\in\left\{ L,R\right\}$ along with the public parameters $\params$.
\item Learner $L$ uses $S_u=\{x_1=(c_{u}^1,\params,y_u^1),\dots ,x_n=(c_{u}^n,\params,y_u^n) \}$ without the $i$th point and $S_v=\{x_1=(c_{v}^1,\params,y_v^1),\dots ,x_n=(c_{v}^n,\params,y_v^n) \}$ without the $i+1$th point with the labels being generated deterministcally by fixing threshold at $N/2$.
\item Sample a random string $r$ for the DP-Learner. Evaluate $h_{r,k_{u},S_{-i}}(c_{u,i})$
and $h_{r,k_{v},S_{-i}}(c_{v,i}).$
\begin{enumerate}
\item if $h_{r,k_{u},S_{-i}}(c_{u,i})=h_{r,k_{v},S_{-i}}(c_{v,i})$, guess
$b=L$
\item if $h_{r,k_{u},S_{-i}}(c_{u,i})\neq h_{r,k_{v},S_{-i}}(c_{v,i})$,
guess $b=R$
\end{enumerate}
\end{enumerate}
\caption{Adversarial strategy using DP-PAC Learner}
\end{algorithm}
\begin{remark}
$m_{i}$ is constructed by removing the set $R_{i}$ from S, where
$\vert R_{i}\vert=O(\log n).$
\end{remark}
\begin{theorem}
Adversary in the security game \ref{alg:game} wins the game with probability at least $\frac{e^{-\epsilon}}{15n^c}$, where $c$ is a constant.
\end{theorem}

\begin{proof}
Let $b'$ denote the guess of the adversary. Let $A_{L}$ denote the
event $h_{r,k_{x,}S_{-i}}(c_{x,i})=h_{r,k_{y},S_{-i}}(c_{y,i})$ and
let $A_{R}$ denote the event $h_{r,k_{x,}S_{-i}}(c_{x,i})\neq h_{r,k_{y},S_{-i}}(c_{y,i})$.
Let $p_{i}=\Pr_{k}\left[h_{k,r,S}(x_{i})=1\right]$

\begin{align*}
\Pr\left[b'=b\right] & =\frac{1}{2}\left(\Pr\left[A_{L}\mid b=L\right]+\Pr\left[A_{R}\mid b=R\right]\right)\\
 & =\frac{1}{2}\left(\frac{1}{2}\left(p_{i}^{2}+(1-p_{i})^{2}+p_{i+1}^{2}+(1-p_{i+1})^{2}\right)+\left(1-p_{i}p_{i+1}-\left(1-p_{i}\right)\left(1-p_{i+1}\right)\right)\right)\\
 & =\frac{1}{2}\left(\frac{1}{2}\left(2p_{i}^{2}+2p_{i+1}^{2}+2-4p_{i}p_{i+1}\right)\right)\\
 & =\frac{1}{2}\left(1+\left(p_{i}-p_{i+1}\right)^{2}\right)
\end{align*}

Using our previous Lemma, we know that for a random string $r,$ $\left(p_{i}-p_{i+1}\right)^{2}\geq\frac{1}{16n^{2}}$
with probability $e^{-\epsilon}/15n^c$. This proves the statement.\rathin{Write about the overall probability is $1/{\poly(n)}$ even if $h$ fails to distinguish}.
\end{proof}






\section{Fixing the bug}

\begin{claim}
There exists an index $i\in [n]$ such that with high probability over $r$,
\begin{align*}
    &\Pr_{k_u,k_v}[h_{r,k_u,S_{-i}}(\Enc(k_u,m_i))=h_{r,k_v,S_{-i}}(\Enc(k_v,m_i))] \\
    -&\Pr_{k_u,k_v}[h_{r,k_u,S_{-i}}(\Enc(k_u,m_{i}))=h_{r,k_v,S_{-i}}(\Enc(k_v,m_{i+1}))]\geq \frac{1}{\poly(n)}
\end{align*}
\end{claim}

Note that both of the probabilities in the above statement are a function of $r$. To simplify notation, we temporarily use $p(r)$ to denote $\Pr_{k_u,k_v}[h_{r,k,S_{-i}}(\Enc(k_u,m_i))=h_{r,k,S_{-i}}(\Enc(k_u,m_i))]$ and use $q(r)$ to denote $\Pr_{k_u,k_v}[h_{r,k,S_{-i}}(\Enc(k_u,m_i))=h_{r,k,S_{-i}}(\Enc(k_u,m_{i+1}))]$.

We analyse the security game now. 

\begin{align*}
\Pr\left[b'=b\right] & =\frac{1}{2}\left(\Pr\left[A_{L}\mid b=L\right]+\Pr\left[A_{R}\mid b=R\right]\right)\\
 & =\frac{1}{2}\left(\expt_r(p(r))+1-\expt_r(q(r))\right)\\
 & = \frac{1}{2}\left(1+\expt_r(p(r))-\expt_r(q(r))\right)
\end{align*}

Since Claim 7.1 holds with high probability, we can argue it holds in expectation thereby getting a polynomial advantage (expectations are not unbounded).

Consider a different analysis for the security game. 

\begin{claim}
There exists an index $i\in [n]$ such that with high probability over $r$,
\begin{align*}
    \Pr_{k}[h_{r,k,S_{-i}}(\Enc(k,m_i))=1]-\Pr_{k}[h_{r,k,S_{-i}}(\Enc(k,m_{i+1}))=1]\geq \frac{1}{\poly(n)}
\end{align*}
\end{claim}

We denote $p_i(r)=\Pr_k[h_{r,k,S_{-i}}(\Enc(k,m_i))=1]$
\begin{align*}
\Pr\left[b'=b\right] & =\frac{1}{2}\left(\Pr\left[A_{L}\mid b=L\right]+\Pr\left[A_{R}\mid b=R\right]\right)\\
 & =\frac{1}{2}\left(\expt_r [p_i]\cdot\expt_r [p_i]+(1-\expt_r[p_i])\cdot(1-\expt_r[p_i])+\expt_r [p_{i+1}]\cdot\expt_r [p_{i+1}]\right)\\
 &+\left(1-\expt_r[p_{i+1}])\cdot(1-\expt_r[p_{i+1}])+ (1-\expt_r[p_i]\expt_{r}[p_{i+1}]-(1-\expt_r[p_i])(1-\expt_r[p_{i+1}]))\right)\\
 &=\frac{1}{2}\left(1+(\expt_r(p_i-p_{i+1}))^2\right)
\end{align*}

We can use the following trick to make a non-negligible probability statement over $r$ instead of a high probability one.

\begin{itemize}
    \item Sample $\Theta$ number of keys uniformly at random.
    \item Generate sets of ciphertexts $C_1,\dots C_{\Theta}$ where $C_i=\{\Enc(k_i,m_1),\dots \Enc(k_i,m_n)\}$ and corresponding $S_i$ where labels are augmented with the $C_i$.
    \item For all $i\in [m], h_{r,k_i,S_i}\gets L(S_i)$
    \item Estimate $\hat{p},\hat{q}$ and get closeness guarantee using Chernoff.
    \item For a bad $r$, guess $b'$ uniformly at random.
\end{itemize}

\begin{claim}
    There exists an index $i\in [n]$ such that with non-neglgible probability over $r$,
\begin{align*}
    \Pr_{k}[h_{r,k,S_{-i}}(\Enc(k,x_i))=1]-\Pr_{k}[h_{r,k,S_{-i}}(\Enc(k,x_{i+1}))=1]\geq \frac{1}{\poly(n)}
\end{align*}
\end{claim}
